GLS-CSC: A Simple but Effective Strategy to Mitigate Chinese STM Models' Over-Reliance on Superficial Clue

Pre-trained models have achieved success in Chinese Short Text Matching (STM) tasks, but they often rely on superficial clues, leading to a lack of robust predictions. To address this issue, it is crucial to analyze and mitigate the influence of superficial clues on STM models. Our study aims to investigate their over-reliance on the edit distance feature, commonly used to measure the semantic similarity of Chinese text pairs, which can be considered a superficial clue. To mitigate STM models' over-reliance on superficial clues, we propose a novel resampling training strategy called Gradually Learn Samples Containing Superficial Clue (GLS-CSC). Through comprehensive evaluations of In-Domain (I.D.), Robustness (Rob.), and Out-Of-Domain (O.O.D.) test sets, we demonstrate that GLS-CSC outperforms existing methods in terms of enhancing the robustness and generalization of Chinese STM models. Moreover, we conduct a detailed analysis of existing methods and reveal their commonality.

==> beifen.tex <==
\begin{table*}[h]
\centering
\resizebox{\linewidth}{!}
{
\begin{tabular}{clcc|cc|ccccc}
\toprule[0.7pt]
\multirow{2}{*}{LCQMC$_{train}$} &            & \multicolumn{2}{c}{\textbf{I.D.}}                                     & \multicolumn{2}{c}{\textbf{Rob.}}                                    & \multicolumn{5}{c}{\textbf{O.O.D.}}                                                                                                                            \\

                          &          & \textbf{LCQMC} & $\Delta$ & \textbf{DUQM} & $\Delta$ & \textbf{OPPO} &  \textbf{BQ} & \textbf{CHC}& \textbf{AVG} & $\Delta$  \\
\midrule[0.5pt]
         \multirow{10}{*}{BERT}                 & Finetune & 86.89\%                               & {-} & 67.19\%                              & {-} & 81.07\%                              & 57.93\%                            & 65.84\%                             & 72.93\%      & {-} \\
                          & Forg.    & 86.49\%                               & -0.40\%              & 68.44\%                              & 1.25\%               & 80.91\%                              & 58.57\%                            & 65.09\%                             & 72.76\%      & -0.17\%              \\
                          & Rew.$_{self}$     & 87.00\%                               & 0.11\%               & 68.41\%                              & 1.22\%               & 80.90\%                              & 57.97\%                            & 65.48\%                             & 72.84\%      & -0.09\%              \\
                          & POE$_{self}$       & 86.77\%                               & -0.12\%              & 65.85\%                              & -1.34\%              & 80.74\%                              & 57.55\%                            & 66.31\%                             & 72.84\%      & -0.09\%              \\
                          & LEAM$_{self}$      & 86.85\%                               & -0.04\%              & 67.35\%                              & 0.16\%               & 80.65\%                              & 58.06\%                            & 66.69\%                             & 73.06\%      & 0.13\%               \\
            \cline{2-11}
                          & Rew.$_{our}$     & 87.74\%                               & 0.85\%               & 69.54\%                              & 2.35\%               & 81.08\%                              & 57.72\%                            & 64.55\%                             & 72.77\%      & -0.16\%              \\
                          & POE$_{our}$       & 88.04\%                               & 1.15\%               & 67.42\%                              & 0.23\%               & 80.74\%                              & 54.99\%                            & 62.96\%                             & 71.68\%      & -1.25\%              \\
                          & LEAM$_{our}$      & 86.97\%                               & 0.08\%               & 68.22\%                              & 1.03\%               & 80.76\%                              & 57.12\%                            & 65.71\%                             & 72.64\%      & -0.29\%              \\
            \cline{2-11}
                          & LLE      & 84.46\%                               & -2.43\%              & 75.52\%                              & 8.33\%               & 79.53\%                              & 61.12\%                            & 69.64\%                             & 73.69\%      & 0.76\%               \\
                       & SULES    & 87.64\%                               & 0.75\%               & 72.32\%                              & 5.13\%               & 81.99\%                              & 58.70\%                            & 67.79\%                             & 74.03\%      & 1.10\%               \\
\midrule[0.5pt]
            \multirow{3}{*}{ERNIE}  & Finetune & 87.46\%                               & {-} & 71.29\%                              & {-} & 82.40\%                              & 60.05\%                            & 66.81\%                             & 74.18\%      & {-} \\
                          & LLE      & 84.02\%                               & -3.44\%              & 77.25\%                              & 5.96\%               & 78.21\%                              & 59.91\%                            & 66.92\%                             & 72.27\%      & -1.92\%              \\
                   & SULES    & 87.61\%                               & 0.15\%               & 75.00\%                              & 3.71\%               & 82.21\%                              & 59.60\%                            & 67.98\%                             & 74.35\%      & 0.17\%               \\
\midrule[0.5pt]
     \multirow{3}{*}{RoBERTa}     & Finetune & 87.56\%                               & {-} & 73.07\%                              & {-} & 82.61\%                              & 60.08\%                            & 68.68\%                             & 74.73\%      & {-} \\
                          & LLE      & 84.82\%                               & -2.74\%              & 79.21\%                              & 6.14\%               & 79.58\%                              & 61.54\%                            & 69.34\%                             & 73.82\%      & -0.91\%              \\
 & SULES    & 87.89\%                               & 0.33\%               & 75.62\%                              & 2.55\%               & 82.68\%                              & 61.23\%                            & 69.14\%                             & 75.24\%      & 0.51\%    \\
\bottomrule[0.7pt]
\end{tabular}
}
% \caption{Experiment on Chinese STM dataset. Train BERT, ERNIE and RoBERTa on LCQMC$_{train}$ with our LLES and SULES method, and evaluate models' ACC (Accuracy) on DuQM$_{test}$, OPPO$_{test}$, GaIIC$_{test}$ and ch-Adset. Besides, we pay attention to AUC (Area under Curve) metric on ch-Adset due to the imbalanced label distribution of ch-Adset. Since the process of sampling with our SULES method is random, R1, R2 and R3 represents different orders of training samples.}
\label{tab:lcqmc_result}
\end{table*}




\begin{table*}[h]
\centering
\resizebox{\linewidth}{!}
{
\begin{tabular}{clcc|cc|ccccc}
\toprule[0.7pt]
\multirow{2}{*}{CCKS$_{train}$} &            & \multicolumn{2}{c}{\textbf{I.D.}}                                     & \multicolumn{2}{c}{\textbf{Rob.}}                                    & \multicolumn{5}{c}{\textbf{O.O.D.}}                                                                                                                            \\

                          &          & \textbf{CCKS} & $\Delta$ & \textbf{DUQM} & $\Delta$ & \textbf{OPPO} &  \textbf{BQ} & \textbf{CHC}& \textbf{AVG} & $\Delta$  \\
\midrule[0.5pt]
         \multirow{10}{*}{BERT}                 & Finetune & 94.13\%                               & {-} & 29.78\%                              & {-} & 49.69\%                              & 84.71\%                            & 70.70\%                             & 74.81\%      & {-} \\
                          & Forg.    & 93.92\%                               & -0.21\%              & 30.45\%                              & 0.67\%               & 50.17\%                              & 84.03\%                            & 69.58\%                             & 74.43\%      & -0.38\%              \\
                          & Rew.$_{self}$     & 93.77\%                               & -0.36\%               & 30.02\%                              & 0.24\%               & 50.70\%                              & 81.67\%                            & 69.85\%                             & 74.00\%      & -0.81\%              \\
                          & POE$_{self}$       & 89.30\%                               & -4.83\%              & 29.53\%                              & -0.25\%              & 49.29\%                              & 83.58\%                            & 69.76\%                             & 72.98\%      & -1.83\%              \\
                          & LEAM$_{self}$      & 92.01\%                               & -2.12\%              & 30.61\%                              & 0.83\%               & 51.06\%                              & 84.01\%                            & 69.43\%                             & 74.13\%      & -0.68\%               \\
            \cline{2-11}
                          & Rew.$_{our}$     & 94.08\%                               & -0.05\%               & 30.31\%                              & 0.53\%               & 51.35\%                              & 84.52\%                            & 71.08\%                             & 75.26\%      & 0.45\%              \\
                          & POE$_{our}$       & 88.27\%                               & -5.86\%               & 29.35\%                              & -0.43\%               & 48.62\%                              & 84.25\%                            & 71.08\%                             & 75.26\%      & 0.45\%              \\
                          & LEAM$_{our}$      & 91.10\%                               & -3.03\%               & 30.47\%                              & 0.69\%               & 49.24\%                              & 84.04\%                            & 70.49\%                             & 73.72\%      & -1.09\%              \\
            \cline{2-11}
                          & LLE      & 76.69\%                               & -17.44\%              & 58.85\%                              & 29.07\%               & 57.84\%                              & 72.57\%                            & 63.90\%                             & 67.75\%      & -7.06\%               \\
                       & SULES    & 93.40\%                               & -0.73\%               & 31.26\%                              & 1.48\%               & 52.32\%                              & 84.73\%                            & 70.42\%                             & 75.22\%      & 0.41\%               \\
\midrule[0.5pt]
            \multirow{3}{*}{ERNIE}  & Finetune & 93.15\%                               & {-} & 33.64\%                              & {-} & 52.76\%                              & 85.61\%                            & 73.76\%                             & 76.32\%      & {-} \\
                          & LLE      & 80.10\%                               & -13.05\%              & 50.74\%                              & 17.10\%               & 60.76\%                              & 76.96\%                            & 70.13\%                             & 71.99\%      & -4.33\%              \\
                   & SULES    & 92.00\%                               & -1.15\%               & 38.17\%                              & 4.53\%               & 57.37\%                              & 85.08\%                            & 74.00\%                             & 77.11\%      & 0.79\%               \\
\midrule[0.5pt]
     \multirow{3}{*}{RoBERTa}     & Finetune & 93.94\%                               & {-} & 32.48\%                              & {-} & 51.85\%                              & 85.57\%                            & 72.20\%                             & 75.89\%      & {-} \\
                          & LLE      & 78.08\%                               & -15.86\%              & 71.67\%                              & 39.19\%               & 68.51\%                              & 73.49\%                            & 64.88\%                             & 71.24\%      & -4.65\%              \\
 & SULES    & 92.78\%                               & -1.16\%               & 39.07\%                              & 6.59\%               & 57.87\%                              & 85.23\%                            & 71.33\%                             & 76.80\%      & 0.91\%    \\
\bottomrule[0.7pt]
\end{tabular}
}
% \caption{Experiment on Chinese STM dataset. Train BERT, ERNIE and RoBERTa on LCQMC$_{train}$ with our LLES and SULES method, and evaluate models' ACC (Accuracy) on DuQM$_{test}$, OPPO$_{test}$, GaIIC$_{test}$ and ch-Adset. Besides, we pay attention to AUC (Area under Curve) metric on ch-Adset due to the imbalanced label distribution of ch-Adset. Since the process of sampling with our SULES method is random, R1, R2 and R3 represents different orders of training samples.}
\label{tab:ccks_result}
\end{table*}

